Precision determination of electroweak parameters and the strange content of the proton from neutrino deep-inelastic scattering

We use recent neutrino dimuon production data combined with a global deep-inelastic parton fit to construct a new parton set, NNPDF1.2, which includes a determination of the strange and antistrange distributions of the nucleon. The result is characterized by a faithful estimation of uncertainties thanks to the use of the NNPDF methodology, and is free of model or theoretical assumptions other than the use of NLO perturbative QCD and exact sum rules. Better control of the uncertainties of the strange and antistrange parton distributions allows us to reassess the determination of electroweak parameters from the NuTeV dimuon data. We perform a direct determination of the |V_cd| and |V_cs| CKM matrix elements, obtaining central values in agreement with the current global CKM fit: specifically we find |V_cd|=0.244\pm 0.019 and |V_cs|=0.96\pm 0.07. Our result for |V_cs| is more precise than any previous direct determination. We also reassess the uncertainty on the NuTeV determination of \sin^2\theta_W through the Paschos-Wolfenstein relation: we find that the very large uncertainties in the strange valence momentum fraction are sufficient to bring the NuTeV result into complete agreement with the results from precision electroweak data.

==> exps-sets.tex <==
 \begin{table}
 \tiny
 \centering
 \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
  \hline
  Experiment & Set & Points & XMIN & XMAX
 & Q2MIN & Q2MAX & STAT (\%)& 
   SYS (\%) & NORM (\%)& TOT (\%) \\ \hline
 NTVDMN   & &  260 & & & & & & & &\\ \hline
 &  NTVnuDMN &   45 &      0.02100 &      0.32600 &        1.127 &      116.467 &  15.8 &   0.0 &   0.0 &  15.8 \\
 \hline
 &  NTVnbDMN &   45 &      0.01500 &      0.20700 &        0.765 &       68.342 &  26.5 &   0.0 &   0.0 &  26.5 \\
 \hline
 \end{tabular}
\caption{}{\small Features of the NuTev dimuon data.\label{tab:exps-sets}}
 \end{table}


==> tab-LHCobs.tex <==
\begin{table}
  \centering
  {\scriptsize
  \begin{tabular}{|c|c|c|c|c|}
    \hline
      &   & $\sigma(W^+){\rm Br}\lp W^+ \to l^+\nu_l\rp\,$ 
          & $\sigma(W^-){\rm Br}\lp W^- \to l^+\nu_l\rp\,$ 
          & $\sigma(Z^0){\rm Br}\lp Z^0 \to l^+l^-\rp\,$ \\
    \hline
    \multirow{2}{*}{NNPDF 1.0} & $10$ TeV &  8.49 $\pm$ 0.18 & 5.81 $\pm$ 0.13 & 1.36 $\pm$ 0.02 \\
                               & $14$ TeV & 11.83 $\pm$ 0.26 & 8.41 $\pm$ 0.20 & 1.95 $\pm$ 0.04 \\
    \hline
    \multirow{2}{*}{NNPDF 1.1} & $10$ TeV &  8.52 $\pm$ 0.33 & 5.79 $\pm$ 0.28 & 1.36 $\pm$ 0.04 \\
                               & $14$ TeV & 11.86 $\pm$ 0.46 & 8.38 $\pm$ 0.39 & 1.95 $\pm$ 0.05 \\
    \hline
    \multirow{2}{*}{NNPDF 1.2} & $10$ TeV &  8.61 $\pm$ 0.25 & 5.85 $\pm$ 0.15 & 1.37 $\pm$ 0.03 \\
                               & $14$ TeV & 11.99 $\pm$ 0.34 & 8.47 $\pm$ 0.21 & 1.97 $\pm$ 0.04 \\
    \hline
  \end{tabular}}
  \caption{}{\small The LHC benchmark cross sections for the present NNPDF1.2
    release, compared to previous releases.\label{tab:LHCobs}}
\end{table}


==> tab_chi2.tex <==
 \begin{table}
 \centering
 \begin{tabular}{|c|c|c|}
  \hline
    &  $N_{\rm dat}$ & $\chi^2$  \\ \hline
NuTeV $\nu+\bar{\nu}$ & 84 & 0.64 \\
NuTeV $\nu$& 43 & 0.60 \\
NuTeV $\bar{\nu}$& 41 & 0.65  \\
 \hline
 \end{tabular}
\caption{}{\small $\chi^2$ for the NuTeV dimuon data,
separated in the neutrino and anti-neutrino samples.
\label{tab:chi2}}
 \end{table}

